Diagnosing Unsupervised RL for Compressing Mathematical Reasoning: Truncation Avoidance and Policy Collapse

Compressing mathematical reasoning within a fixed response budget is a practical but underexplored setting, where responses that reach the generation limit without an EOS token are incomplete. We study whether unsupervised reinforcement learning (RL) with intrinsic lengthand entropy-based rewards can improve this fixed-budget outcome. We operationalize compression through truncation avoidance: the EOS-verified truncation rate decreases while mathematical accuracy is maintained or improved. Across four Large Language Models (LLMs), a direct length penalty (LP) and a cumulative token-entropy penalty (Ent) can produce a transient compression regime before policy collapse. Across the evaluated models, higher baseline mathematical performance is generally associated with a longer regime and later collapse. We further cluster tokenentropy trajectories to construct a responselevel entropy space. The expansion rate of its explored region increases near policy collapse, with generally later and smaller increases for models with higher baseline mathematical performance.

==> review.tex <==
\def\bluereview{1}
\input{eacl_meta_revised.tex}

